COAST: Enhancing the Code Debugging Ability of LLMs through Communicative Agent Based Data Synthesis

Code debugging is a vital stage of software development, essential for ensuring the reliability and performance of Large Language Models (LLMs) in the code generation task. Human debugging typically follows a multi-stage process, which includes Bug Localization, Bug Identification, Code Repair, and Code Recognition. However, existing code debugging benchmarks predominantly focus on the Code Repair stage, which offers only a limited perspective on evaluating the debugging capabilities of LLMs. In this paper, we introduce DEBUGEVAL, a comprehensive benchmark for evaluating the debugging abilities of LLMs by emulating the multi-stage human debugging process. Through evaluating on DEBUGEVAL, we observe that 7B-scale models consistently underperform compared to their larger counterparts, highlighting their limitations in comprehending code semantics. In this case, we propose the COmmunicative Agent-based data SynThesis (COAST) framework, which employs a multi-agent system to generate high-quality training data for supervised fine-tuning (SFT). Experimental results demonstrate that COAST-generated data outperform human-curated and GPT-4-generated data, enabling 7B-scale LLMs to achieve debugging performance comparable to GPT-3.5. All data and codes are available at https://github.com/NEUIR/COAST.

==> tables/comparision.tex <==
\begin{table*}[t]
\small
\centering
\caption{A Comparison between \benchmark and Other Code Repair Benchmarks. The data statistics only on the testing set of each benchmark. CE indicates compilation errors (e.g. SyntaxError). The Source indicates where the buggy codes are collected.}
\label{tab:comparision}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllrccc}
\hline
\textbf{Dataset} & \textbf{Language} & \textbf{Task}                                                                                            & \textbf{Size}                                                     & \textbf{Type} & \textbf{Source} &\textbf{Anti-Data Leakage} \\ \hline
DeepFix~\citeyearpar{yasunaga2021break}          & C                 & Code Repair                                                                                               & 6,971                                                           & CE     &   User         & \textcolor{red}{\ding{55}}   \\
Review4Repair~\citeyearpar{huq2022review4repair}    & Java              & Code Repair                                                                                               & 2,961                                                              & All     &   User             & \textcolor{red}{\ding{55}}   \\
Bug2Fix~\citeyearpar{lu2021codexglue}          & Java              & Code Repair                                                                                               & 5,835                                                              & All    &  User               & \textcolor{red}{\ding{55}}   \\
Github-Python~\citeyearpar{yasunaga2021break}        & Python            & Code Repair                                                                                               & 15K                                                               & CE  &   User            & \textcolor{red}{\ding{55}}   \\
FixEval~\citeyearpar{haque2023fixeval}          & Java/Python       & Code Repair                                                                                               & 43K/243K                                                           & All   &   User               & \textcolor{red}{\ding{55}}   \\
CodeError~\citeyearpar{wang2024intervenor}        & Python            & Code Repair                                                                                               & 4,463                                                              & All   &    User              & \textcolor{red}{\ding{55}}   \\
DebugBench~\citeyearpar{tian2024debugbench}       & C++/Java/Python   & Code Repair                                                                                               & 1,438/1,401/1,414& All    &    GPT-4              & \textcolor{green}{\ding{51}}     \\
CodeEditorBench~\citeyearpar{guo2024codeeditorbench}  & C++/Java/Python   & Code Repair                                                                                               & 676/515/716& All      & GPT-4              & \textcolor{green}{\ding{51}}     \\ \hline
\benchmark   & C++/Java/Python   & \begin{tabular}[c]{@{}l@{}}BUG Localization\\ BUG Identification\\ Code Review\\ Code Repair\end{tabular} & \begin{tabular}[c]{@{}r@{}}195/205/178\\ 800/760/760\\  800/800/800\\ 138/138/138\\\end{tabular}&  All    &    \begin{tabular}[c]{@{}c@{}}User \\ GPT-4  \end{tabular}             & \textcolor{green}{\ding{51}}     \\ \hline
\end{tabular}
}
\end{table*}

==> tables/data_quantity_experiment.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\caption{Performance of Different Data Quantity.}
\label{tab:Analysis 2}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|ccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multirow{2}{*}{\textbf{Quantity}} & \multicolumn{5}{c}{\textbf{Task}} \\ \cline{3-7} 
\multicolumn{1}{c|}{} &  & \textbf{BUG Loc.} & \textbf{BUG Iden.} & \textbf{Code Rec.} & \textbf{Code Rep.} & \textbf{Avg.} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}DSCoder-6.7B-Ins\\ (w/ Mixed Strateg)\end{tabular}} & 0 & 27.5 & 26.2 & 20.3 & 40.6 & 28.7 \\
 & 5K & 39.3 & 30.1 & 54.7 & 45.4 & 42.4 \\
 & 10K & 49.3 & 38.2 & 33.3 & 43.7 & 41.1 \\
 & 15K & 51.9 & 40.9 & 48.8 & 46.4 & 47.0 \\
 & 20K & 55.2 & 39.4 & 66.0 & 48.3 & 52.2 \\
 & 25K & \textbf{58.8} & \textbf{45.8} & \textbf{71.3} & \textbf{49.5} & \textbf{56.4} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Llama3-8B-Ins\\ (w/ Mixed Strategy)\end{tabular}} & 0 & 57.6 & 36.6 & 74.9 & 29.6 & 49.7 \\
 & 5K & 60.9 & \textbf{40.9} & 67.3 & 39.6 & 52.2 \\
 & 10K & \textbf{61.4} & 37.9 & 78.9 & 40.8 & \textbf{54.8} \\
 & 15K & 60.9 & 35.7 & 78.0 & 40.8 & 53.9 \\
 & 20K & 60.7 & 36.0 & \textbf{79.1} & 41.1 & 54.2 \\
 & 25K & 61.1 & 33.8 & 78.5 & \textbf{41.8} & 53.8 \\ \hline
\end{tabular}
}
\end{table}

==> tables/data_statistics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\small
\centering
\caption{Data Statistics of \benchmark.}
\label{tab:data_statistics}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{l|c|r}
\hline
\textbf{Evaluation Tasks}                                                                                                                       & \multicolumn{1}{r|}{\textbf{Language}} & \textbf{\#Test} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{BUG Localization}: Identify which code fragm-\\ ent in the buggy code causing the error.\end{tabular}} & Python                                 & 178           \\
                                                                                                                                                   & C++                                    & 195           \\
                                                                                                                                                   & Java                                   & 205           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{BUG Identification}: Identify the type of error\\  in your code.\end{tabular}}                            & Python                                 & 760           \\
                                                                                                                                                   & C++                                    & 800           \\
                                                                                                                                                   & Java                                   & 760           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Code Review}: Determine which code is incor-\\ rect.\end{tabular}}                                        & Python                                 & 800           \\
                                                                                                                                                   & C++                                    & 800           \\
                                                                                                                                                   & Java                                   & 800           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Code Repair}: Fixing the buggy code to passes \\ all the test cases.\end{tabular}}                        & Python                                 & 138           \\
                                                                                                                                                   & C++                                    & 138           \\
                                                                                                                                                   & Java                                   & 138           \\ \hline
\end{tabular}
}
\end{table}

==> tables/differnet_benchs_compare.tex <==
\begin{table*}[]
\small
\centering
\caption{Result of the DebugEval Comparison with Other Benchmarks.}
\label{tab:different benchs}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|ccccc}
\hline
\multicolumn{1}{c|}{BenchMark} & Debug Task Diversity & Language Diversity & Avoid Data Leakage & Bug Type Diversity & Test Scale \\ \hline
QuixBugs & \times & \times & \times & \times & 40 \\
LiveCode & \times & \times & \checkmark & \checkmark & 500 \\
CodeError & \times & \times & \checkmark & \checkmark & 4463 \\
CodeEdit  & \times & \checkmark & \checkmark & \checkmark & 1907 \\
DebugBench & \times & \checkmark & \checkmark & \checkmark & 4253 \\ \hline
DebugEval  & \checkmark & \checkmark & \checkmark & \checkmark & 5712 \\ \hline
\end{tabular}
}
\end{table*}


